LLMODE: Aligning ODEs with LLMs via Gated Token Injection for Irregular Spatio-Temporal Forecasting

Large language models (LLMs) have shown promise for spatio-temporal forecasting, but existing approaches often rely on regularly sampled token sequences and struggle with irregular observations because of temporal asynchrony, representation-space misalignment, and limited context windows. We propose LLMODE, a token-efficient framework for irregular spatio-temporal forecasting with a frozen LLM backbone. LLMODE first uses a graph-aware ODE encoder to reconstruct irregular graph observations as a continuous-time latent trajectory. A Fixed-Budget Perceiver Resampler then compresses this variable-length trajectory into a fixed number of dynamic memory tokens. In parallel, compact statistical descriptors are encoded and resampled into context memory tokens. A dual-source gated cross-attention module injects both memories into the frozen LLM, enabling controlled utilization of external spatio-temporal evidence. Experiments on three real-world urban datasets and two physical-dynamics benchmarks show competitive overall performance, with clearer advantages under sparse or dynamically complex irregular sampling. Additional evaluations on unseen urban regions further demonstrate strong zero-shot generalization without adaptation.

==> table/table_main_with_std.tex <==
% Required packages in the main document:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
%
% Existing project commands are also required:
% \model
% \secondbest

\begin{table*}[t]
\centering
\scriptsize
\caption{Main results on NYC and physics benchmarks, measured by MAE and MSE. Average results on $5$ independent runs are reported. $*$ indicates statistically significant improvements over the best baseline, with $p$-value smaller than $0.001$.}
\label{tab:main_results}
\vspace{-4pt}

\textbf{(a) Results on NYC benchmarks.}\par
\vspace{2pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{3}{*}{Method}
& \multicolumn{4}{c}{NYCtaxi}
& \multicolumn{4}{c}{NYCbike}
& \multicolumn{4}{c}{NYCcrime} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
& \multicolumn{2}{c}{inflow}
& \multicolumn{2}{c}{outflow}
& \multicolumn{2}{c}{inflow}
& \multicolumn{2}{c}{outflow}
& \multicolumn{2}{c}{robbery}
& \multicolumn{2}{c}{burglary} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\cmidrule(lr){6-7}\cmidrule(lr){8-9}
\cmidrule(lr){10-11}\cmidrule(lr){12-13}
& MAE & MSE & MAE & MSE
& MAE & MSE & MAE & MSE
& MAE & MSE & MAE & MSE \\
\midrule
TGCN & 0.1145$_{\pm0.0011}$ & 0.0367$_{\pm0.0006}$ & 0.0875$_{\pm0.0006}$ & 0.0331$_{\pm0.0007}$ & 0.2211$_{\pm0.0024}$ & 0.1572$_{\pm0.0032}$ & 0.1506$_{\pm0.0014}$ & 0.0657$_{\pm0.0013}$ & 0.9970$_{\pm0.0126}$ & 1.0849$_{\pm0.0218}$ & 0.6746$_{\pm0.0040}$ & 1.0029$_{\pm0.0188}$ \\
STSGCN & 0.0847$_{\pm0.0010}$ & 0.0286$_{\pm0.0004}$ & 0.0704$_{\pm0.0006}$ & 0.0349$_{\pm0.0004}$ & 0.1951$_{\pm0.0006}$ & 0.1734$_{\pm0.0019}$ & 0.1669$_{\pm0.0021}$ & 0.1119$_{\pm0.0020}$ & 0.9162$_{\pm0.0151}$ & 1.5371$_{\pm0.0272}$ & 0.6293$_{\pm0.0110}$ & 0.8300$_{\pm0.0206}$ \\
MTGNN & 0.0371$_{\pm0.0005}$ & 0.0143$_{\pm0.0002}$ & 0.0337$_{\pm0.0002}$ & 0.0365$_{\pm0.0003}$ & \secondbest{0.0786$_{\pm0.0015}$} & \secondbest{0.0263$_{\pm0.0004}$} & \secondbest{0.0824$_{\pm0.0005}$} & \secondbest{0.0265$_{\pm0.0005}$} & 0.8252$_{\pm0.0081}$ & 1.1408$_{\pm0.0138}$ & 0.6283$_{\pm0.0044}$ & 0.7857$_{\pm0.0136}$ \\
BiTGraph & 0.0731$_{\pm0.0007}$ & 0.0305$_{\pm0.0003}$ & 0.0540$_{\pm0.0009}$ & 0.0301$_{\pm0.0008}$ & 0.0837$_{\pm0.0009}$ & 0.0298$_{\pm0.0008}$ & 0.0830$_{\pm0.0015}$ & 0.0275$_{\pm0.0006}$ & 0.8555$_{\pm0.0100}$ & 1.2376$_{\pm0.0083}$ & 0.5321$_{\pm0.0082}$ & 0.4988$_{\pm0.0147}$ \\
FourierGNN & 0.1234$_{\pm0.0020}$ & 0.0246$_{\pm0.0005}$ & 0.1026$_{\pm0.0010}$ & 0.0187$_{\pm0.0002}$ & 0.1533$_{\pm0.0011}$ & 0.0734$_{\pm0.0007}$ & 0.1523$_{\pm0.0018}$ & 0.0626$_{\pm0.0010}$ & 0.4074$_{\pm0.0040}$ & 0.8993$_{\pm0.0077}$ & 0.2666$_{\pm0.0026}$ & 0.2899$_{\pm0.0023}$ \\
\midrule
ISTS-PLM & \textbf{0.0329$_{\pm0.0003}$} & \secondbest{0.0068$_{\pm0.0001}$} & 0.0263$_{\pm0.0003}$ & \secondbest{0.0059$_{\pm0.0001}$} & 0.1061$_{\pm0.0012}$ & 0.0461$_{\pm0.0009}$ & 0.1077$_{\pm0.0014}$ & 0.0488$_{\pm0.0013}$ & 0.4271$_{\pm0.0046}$ & 0.4055$_{\pm0.0107}$ & 0.3040$_{\pm0.0044}$ & 0.2143$_{\pm0.0036}$ \\
UrbanGPT & 0.0359$_{\pm0.0004}$ & 0.0080$_{\pm0.0001}$ & \secondbest{0.0262$_{\pm0.0003}$} & 0.0068$_{\pm0.0001}$ & 0.0787$_{\pm0.0007}$ & 0.0301$_{\pm0.0007}$ & 0.0833$_{\pm0.0004}$ & 0.0292$_{\pm0.0002}$ & 0.9336$_{\pm0.0088}$ & 1.7088$_{\pm0.0226}$ & 0.6192$_{\pm0.0088}$ & 0.8341$_{\pm0.0146}$ \\
GPT4TS & 0.0424$_{\pm0.0006}$ & 0.0260$_{\pm0.0006}$ & 0.0312$_{\pm0.0006}$ & 0.0209$_{\pm0.0005}$ & 0.1592$_{\pm0.0024}$ & 0.2072$_{\pm0.0043}$ & 0.1636$_{\pm0.0011}$ & 0.2129$_{\pm0.0027}$ & 0.3350$_{\pm0.0029}$ & 0.2578$_{\pm0.0026}$ & \secondbest{0.2398$_{\pm0.0032}$} & 0.1229$_{\pm0.0030}$ \\
\midrule
GRU-ODE & 0.0956$_{\pm0.0016}$ & 0.0645$_{\pm0.0015}$ & 0.0708$_{\pm0.0009}$ & 0.0607$_{\pm0.0017}$ & 0.3100$_{\pm0.0006}$ & 0.4081$_{\pm0.0024}$ & 0.3443$_{\pm0.0043}$ & 0.4964$_{\pm0.0179}$ & 0.3678$_{\pm0.0030}$ & 0.4161$_{\pm0.0095}$ & 0.2483$_{\pm0.0028}$ & 0.1815$_{\pm0.0025}$ \\
tPatchGNN & 0.0338$_{\pm0.0005}$ & 0.0082$_{\pm0.0000}$ & 0.0347$_{\pm0.0003}$ & 0.0095$_{\pm0.0002}$ & 0.0800$_{\pm0.0008}$ & 0.0476$_{\pm0.0008}$ & 0.0849$_{\pm0.0007}$ & 0.0484$_{\pm0.0006}$ & \secondbest{0.3052$_{\pm0.0070}$} & \secondbest{0.1428$_{\pm0.0017}$} & 0.2483$_{\pm0.0046}$ & \secondbest{0.1119$_{\pm0.0022}$} \\
ViTST & 0.3548$_{\pm0.0031}$ & 0.1718$_{\pm0.0010}$ & 0.2938$_{\pm0.0035}$ & 0.1377$_{\pm0.0031}$ & 0.4371$_{\pm0.0032}$ & 0.6891$_{\pm0.0170}$ & 0.4542$_{\pm0.0070}$ & 0.7136$_{\pm0.0076}$ & 0.4582$_{\pm0.0037}$ & 0.5084$_{\pm0.0103}$ & 0.3267$_{\pm0.0033}$ & 0.2325$_{\pm0.0047}$ \\
\midrule
\textbf{\model} & \secondbest{0.0336$_{\pm0.0007}$} & \textbf{0.0066$_{\pm0.0001}$} & \textbf{0.0252$_{\pm0.0002}$} & \textbf{0.0057$_{\pm0.0001}$} & \textbf{0.0767$_{\pm0.0008}$}$^*$ & \textbf{0.0243$_{\pm0.0003}$}$^*$ & \textbf{0.0817$_{\pm0.0010}$} & \textbf{0.0242$_{\pm0.0005}$}$^*$ & \textbf{0.3050$_{\pm0.0031}$} & \textbf{0.1396$_{\pm0.0011}$}$^*$ & \textbf{0.2394$_{\pm0.0029}$} & \textbf{0.0790$_{\pm0.0016}$}$^*$ \\
\bottomrule
\end{tabular}%
}

\vspace{7pt}

\textbf{(b) Results on physics benchmarks.}\par
\vspace{2pt}
\resizebox{0.78\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\toprule
\multirow{3}{*}{Method}
& \multicolumn{4}{c}{Springs}
& \multicolumn{4}{c}{Charged} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
& \multicolumn{2}{c}{X}
& \multicolumn{2}{c}{Y}
& \multicolumn{2}{c}{X}
& \multicolumn{2}{c}{Y} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\cmidrule(lr){6-7}\cmidrule(lr){8-9}
& MAE & MSE & MAE & MSE
& MAE & MSE & MAE & MSE \\
\midrule
TGCN & 0.1971$_{\pm0.0026}$ & 0.0741$_{\pm0.0011}$ & 0.1934$_{\pm0.0020}$ & 0.0708$_{\pm0.0008}$ & 0.4706$_{\pm0.0044}$ & 0.3038$_{\pm0.0048}$ & 0.4710$_{\pm0.0112}$ & 0.3042$_{\pm0.0054}$ \\
STSGCN & 0.3306$_{\pm0.0035}$ & 0.1686$_{\pm0.0036}$ & 0.3114$_{\pm0.0036}$ & 0.1754$_{\pm0.0037}$ & 0.3804$_{\pm0.0053}$ & 0.2153$_{\pm0.0008}$ & 0.4152$_{\pm0.0031}$ & 0.2879$_{\pm0.0064}$ \\
MTGNN & \secondbest{0.1053$_{\pm0.0024}$} & \secondbest{0.0237$_{\pm0.0003}$} & \secondbest{0.1086$_{\pm0.0006}$} & \secondbest{0.0249$_{\pm0.0009}$} & \secondbest{0.1410$_{\pm0.0017}$} & 0.0533$_{\pm0.0007}$ & 0.1482$_{\pm0.0024}$ & 0.0535$_{\pm0.0012}$ \\
BiTGraph & 0.1271$_{\pm0.0007}$ & 0.0312$_{\pm0.0004}$ & 0.1290$_{\pm0.0007}$ & 0.0321$_{\pm0.0004}$ & 0.1501$_{\pm0.0015}$ & 0.0578$_{\pm0.0007}$ & 0.1527$_{\pm0.0013}$ & 0.0593$_{\pm0.0005}$ \\
FourierGNN & 0.2108$_{\pm0.0015}$ & 0.0767$_{\pm0.0018}$ & 0.2127$_{\pm0.0036}$ & 0.0788$_{\pm0.0012}$ & 0.2305$_{\pm0.0033}$ & 0.1000$_{\pm0.0015}$ & 0.2309$_{\pm0.0044}$ & 0.1003$_{\pm0.0025}$ \\
\midrule
ISTS-PLM & 0.1513$_{\pm0.0017}$ & 0.0427$_{\pm0.0005}$ & 0.1505$_{\pm0.0012}$ & 0.0423$_{\pm0.0008}$ & 0.1524$_{\pm0.0010}$ & 0.0569$_{\pm0.0010}$ & 0.1539$_{\pm0.0030}$ & 0.0576$_{\pm0.0014}$ \\
UrbanGPT & 0.1519$_{\pm0.0021}$ & 0.0420$_{\pm0.0005}$ & 0.1514$_{\pm0.0016}$ & 0.0424$_{\pm0.0008}$ & 0.1633$_{\pm0.0029}$ & 0.0702$_{\pm0.0005}$ & 0.1746$_{\pm0.0015}$ & 0.0908$_{\pm0.0007}$ \\
GPT4TS & 0.4549$_{\pm0.0082}$ & 0.2826$_{\pm0.0073}$ & 0.4549$_{\pm0.0020}$ & 0.2838$_{\pm0.0060}$ & 0.4996$_{\pm0.0073}$ & 0.3447$_{\pm0.0086}$ & 0.5009$_{\pm0.0051}$ & 0.3469$_{\pm0.0064}$ \\
\midrule
GRU-ODE & 0.3132$_{\pm0.0028}$ & 0.1664$_{\pm0.0023}$ & 0.3080$_{\pm0.0037}$ & 0.1615$_{\pm0.0030}$ & 0.3001$_{\pm0.0061}$ & 0.1543$_{\pm0.0042}$ & 0.2888$_{\pm0.0027}$ & 0.1399$_{\pm0.0006}$ \\
tPatchGNN & 0.1391$_{\pm0.0021}$ & 0.0370$_{\pm0.0008}$ & 0.1384$_{\pm0.0010}$ & 0.0367$_{\pm0.0006}$ & 0.1439$_{\pm0.0009}$ & \secondbest{0.0504$_{\pm0.0008}$} & \secondbest{0.1497$_{\pm0.0022}$} & \secondbest{0.0504$_{\pm0.0003}$} \\
ViTST & 0.4519$_{\pm0.0018}$ & 0.2751$_{\pm0.0053}$ & 0.4524$_{\pm0.0043}$ & 0.2767$_{\pm0.0074}$ & 0.4842$_{\pm0.0030}$ & 0.3174$_{\pm0.0068}$ & 0.4849$_{\pm0.0086}$ & 0.3181$_{\pm0.0040}$ \\
\midrule
\textbf{\model} & \textbf{0.0973$_{\pm0.0016}$}$^*$ & \textbf{0.0191$_{\pm0.0004}$}$^*$ & \textbf{0.0986$_{\pm0.0010}$}$^*$ & \textbf{0.0196$_{\pm0.0003}$}$^*$ & \textbf{0.1402$_{\pm0.0028}$} & \textbf{0.0483$_{\pm0.0002}$}$^*$ & \textbf{0.1461$_{\pm0.0024}$}$^*$ & \textbf{0.0493$_{\pm0.0002}$}$^*$ \\
\bottomrule
\end{tabular}%
}

\end{table*}

